Optimal Diamond Distance Estimation for Unitary Channels

The diamond distance between two quantum channels determines the optimal probability of distinguishing them from a single use. We give a quantum algorithm that estimates the diamond distance between two unknown $d$-dimensional unitary channels to within additive error $\varepsilon$, using $O(\sqrt{d}/\varepsilon)$ queries to the unitary channels and their inverses. The query complexity is optimal, as it matches the lower bound due to Jeon and Oh (npj Quantum Inf. 2026).

==> geometry_style.tex <==
% Shared physical dimensions and styles for the manuscript's geometry figures.
% Load inside each figure's group so these names remain local.
\definecolor{figureblue}{RGB}{0,91,150}
\definecolor{figureorange}{RGB}{184,76,0}

\def\figRadius{1.40}
\def\figAngleRadius{0.65}
\def\figCapRadius{0.40}
\def\figIntervalRadius{1.65}
\def\figOriginRadius{0.8pt}
\def\figWidth{16.1}
\def\figLeftX{3.30}
\def\figRightX{12.10}
\def\figMiddleX{8.05}
\def\figCenterY{3.25}
\def\figTitleY{5.88}
\def\figTopY{6.20}

\tikzset{
  geometry figure/.style={x=1cm,y=1cm,font=\small,>=stealth},
  circle outline/.style={draw=black!55,line width=0.65pt},
  coordinate axis/.style={draw=black!35,line width=0.45pt,->},
  axis label/.style={text=black!60,font=\footnotesize,inner sep=2pt},
  panel title/.style={font=\small\bfseries},
  legend label/.style={font=\footnotesize,inner sep=0pt},
  short arc/.style={draw=figureblue,line width=1.5pt},
  containing arc/.style={short arc},
  phase interval/.style={draw=black!65,dashed,line width=0.9pt},
  point/.style={circle,fill=black,inner sep=1.6pt},
  spectral point/.style={point},
  reference point/.style={circle,fill=figureorange,inner sep=2.2pt},
  antipode point/.style={circle,draw=figureorange,fill=white,line width=0.9pt,inner sep=2.0pt},
  cut point/.style={circle,draw=black!65,fill=white,line width=0.8pt,inner sep=1.8pt},
  origin fill/.style={fill=black!60},
  label guide/.style={draw=black!50,line width=0.45pt},
  blue label guide/.style={label guide,draw=figureblue},
  orange label guide/.style={label guide,draw=figureorange},
  radius guide/.style={draw=black!35,densely dotted,line width=0.6pt},
  diameter guide/.style={radius guide,draw=figureorange!45},
  angle measure/.style={draw=figureblue,line width=0.65pt},
  angle arc/.style={angle measure,->},
  capped angle/.style={draw=figureorange,line width=0.9pt,->},
  rotation arrow/.style={draw=black!65,line width=0.8pt,->}
}

\newcommand{\figureAxes}{%
  \draw[coordinate axis] (-1.85,0) -- (1.95,0)
    node[axis label,above right] {$\operatorname{Re}$};
  \draw[coordinate axis] (0,-1.75) -- (0,1.95)
    node[axis label,above right] {$\operatorname{Im}$};
  \draw[circle outline] (0,0) circle[radius=\figRadius];
}

% Legend entries share a column grid at the bottom of each figure.
% Arguments: style, column x, row y, text.
\def\legendColA{1.00}
\def\legendColB{5.20}
\def\legendColC{9.90}
\def\legendRowA{0.80}
\def\legendRowB{0.30}
\newcommand{\legendMarker}[4]{%
  \node[#1] at ({#2+0.3},#3) {};
  \node[anchor=west,legend label] at ({#2+0.75},#3) {#4};
}
\newcommand{\legendLine}[4]{%
  \draw[#1] (#2,#3) -- ({#2+0.6},#3);
  \node[anchor=west,legend label] at ({#2+0.75},#3) {#4};
}

